The Circumbilliard: Any Triangle can be a 3-Periodic

A Circumconic passes through a triangle's vertices. We define the Circumbilliard, a circumellipse to a generic triangle for which the latter is a 3-periodic. We study its properties and associated loci.

==> _not_used/050_circumellipses.tex <==
The Medial Triangle divides the plane in 7 regions, see  Figure~\ref{fig:midlines}. The following is a known fact  \cite{akopyan2007-conics,odehnal2015-conics}:

\begin{remark}
If the center of a Circumconic lies within 4 of these (resp. the remainder 3), the conic will be an Ellipse (resp. Hyperbola).
\end{remark}

\begin{figure}
    \centering
    % used inkspace to go from .pdf -> .eps
    \includegraphics[width=\textwidth]{pics_eps_new/0070_medial_midlines_cropped.eps}
    \caption{A reference triangle is shown (blue) as well as its Medial (red). The latter sides divide the plane into 7 regions, including the Medial' s interior. When a Circumconic center lies on any of the shaded regions (resp. unshaded) it is an Ellipse (resp. Hyperbola). Parabolas have centers at infinity. For illustration, the $X_1$ and $X_9$-centered Circumellipses and the $X_{11}$-centered Feuerbach Hyperbola are shown. Note that over the family of 3-periodics, a given Circumconic may alternate between Ellipse and Hyperbola, e.g., when centered on $X_4$, $X_5$, $X_6$, etc.}
    \label{fig:midlines}
\end{figure}

Centers $X_1$, $X_2$, and $X_9$ are always interior to the Medial Triangle \cite{etc}, so the Circumconics $E_i,i=1,2,9$ centered on them will ellipses, Figure~\ref{fig:circumX1X2}. $E_2$ is the {\em Steiner Circumellipse}, least-area over all possible Circumellipses \cite{mw}, and $E_9$ is $T$'s CB, see Section~\ref{sec:cb}.

It is known that $E_1$ intersects the EB and the Circumcircle at $X_{100}$, the Anticomplement of the Feuerbach Point. Also that $E_2$ intersects $E_9$ at $X_{190}$, the Yff Parabolic Point \cite{dekov14,etc}. These two ellipses intersect at $X_{664}$\footnote{This is the isogonal conjugate of $X_{663}$, i.e., $\mathcal{L}_{663}$ mentioned before is coincidentally its {\em Trilinear Polar} \cite{mw}.} \cite{moses2020-private-circumconic}.

Given a generic triangle $T$:

\begin{proposition}
The axes of $E_1$  are parallel to $E_9$'s. %${e_1}{e_2}={-a^2+2+2\delta}{a^4(2 a^2-1+2\delta)}$.
\end{proposition}

The proof is in Appendix~\ref{app:circum-x1x2x9}. 

\begin{theorem}
Over the 3-periodic family, the major $\eta_1'$ (resp. minor $\eta_1$) semiaxis lengths of $E_1$ are variable, though their ratio is invariant. These are given by:

\begin{align*}
\eta_1'=&R+d,\;\;\;\eta_1=R-d\\ 
\frac{\eta_1'}{\eta_1}
%&=\frac{\sqrt{2\delta^2+2(a^2-b^2)\delta-a^2b^2}}{b^2} \\
=&\frac{R+d}{R-d}=\frac{1+\sqrt{1-2\rho}}{\rho}-1 > 1
\end{align*}
\label{thm:axis-ratio}
\end{theorem}
\noindent Where $d=|X_1X_3|=\sqrt{R(R-2r)}$.

%\begin{equation}
%\label{eqn:rovR}
%\frac{r}{R}=\frac{2(\delta-b^2)(a^2-\delta)}{(a^2-b^2)^2}
%\end{equation}

\begin{proof}
Calculate the ratio using vertex locations (see \cite{garcia2020-new-properties}) for an isosceles orbit, and then verify with a Computer Algebra System (CAS) the expression holds over the entire family. A related proof appears in \cite{reznik2020-poristic}.
\end{proof}

Note: experimentally $\eta_1'$ is maximal (resp. minimal) when the 3-periodic is an isosceles with axis of symmetry parallel to the EB's minor (resp. major) axis.

\begin{proposition}
The axes of $E_2$ are only parallel to $E_9$ if $T$ is isosceles.
\end{proposition}

See Appendix~\ref{app:circum-x1x2x9}.

%\begin{observation}
%The intersection of %$E_1$ and $E_2$ which is %not a vertex of $T$ is %collinear with $X_{75}$ %and $X_{77}$.
%\end{observation}


% \begin{observation}
%$E_2$ axes are only parallel to the EB's when orbits are isosceles triangles (4 discrete cases). Their lengths $\eta_2$ and $\eta_2'$ are related as $\eta_2 = c_0 + c_1 \eta_2'$, with $c_0,c_1$ constant for all orbits. \textcolor{red}{ronaldo consegue derivar $c_0$ e $c_1$?}
%\end{observation}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0091_e1e2.eps}
    \caption{$E_1$ (green) and $E_2$ (brown) are Circumellipses to the orbit (blue) centered on $X_1$ (green) and $X_2$ (brown). The former (resp.~latter) intersect the EB at $X_{100}$ (resp.~$X_{190}$). They intersect at the vertices and at $X_{664}$. $E_1$ axes remain parallel to the EB over the orbit family, and the ratio of their lengths is constant. The axes of $E_2$ are only parallel to the EB's when the orbit is an isosceles. \textbf{Video}: \cite[PL\#08]{reznik2020-playlist-circum}.}
    \label{fig:circumX1X2}
\end{figure}

\subsection{Parallel-Axis Pencil}

The Feuerbach Circumhyperbola of a Triangle is a rectangular hyperbola\footnote{Since it passes through the Orthocenter $X_4$ \cite{mw}.} centered on $X_{11}$ \cite{mw}.
Peter Moses has contributed a stronger generalization \cite{moses2020-private-circumconic}:

\begin{remark}
The pencil of Circumconics whose centers lie on the Feuerbach Circumhyperbola $F_{med}$ of the Medial Triangle have mutually-parallel axes. 
\end{remark}

The complement\footnote{The 2:1 reflection of a point about $X_2$.} of $X_{11}$ is $X_{3035}$ \cite{etc} so $F_{med}$ is centered there, see Figure~\ref{fig:circum_parallel}. The following is a list of Circumellipses whose centers lie on $F_{med}$ \cite{moses2020-private-circumconic}: $X_i$,  $i$=1, 3, 9, 10\footnote{Notice $X_{10}$ is the Incenter of the Medial. Interestingly, $X_8$, the Incenter of the ACT, does not belong to this select group.}, 119, 142, 214, 442, 600, 1145, 2092, 3126, 3307, 3308, 3647, 5507, 6184, 6260, 6594, 6600, 10427, 10472, 11517, 11530, 12631, 12639, 12640, 12864, 13089, 15346, 15347, 15348, 17057, 17060, 18258, 18642, 19557, 19584, 22754, 34261, 35204.
%The  results below have been observed experimentally, but still lack a proof.

\begin{proposition}
\label{th:9}
A circumellipse has  center on $F_{med}$ iff it passes through $X_{100}$.
\end{proposition}

A proof appears in Appendix~\ref{app:ce_parallel}. The following has been observed experimentally:

\begin{conjecture}
Over the family of 3-periodics, all Circumellipses in Moses' pencil conserve the ratio of their axes.
\label{conj:moses}
\end{conjecture}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0050_ce_x100.eps}
    \caption{An $a/b=1.5$ EB is shown (black) centered on $X_9$ as well as a sample 3-periodic (blue). Also shown are Circumellipses centered on $X_i$, $i=$1, 3, 10, 142, whose centers lie on the Feuerbach Circumhyperbola of the Medial Triangle (both shown red), centered on $X_{3035}$, the complement of $X_{11}$. Notice all conics drawn (including the Circumhyp). have axes parallel to the EB and all Circumellipses pass through $X_{100}$. Note: the Circumellipse centered on $X_3$ is the Circumcircle, its axes, drawn diagonally, are immaterial.}
    \label{fig:circum_parallel}
\end{figure}

==> _not_used/060_circumhyperbolae.tex <==

Here we study invariants of two well-known Circumhyperbolae\footnote{Its centers lie in the unshaded regions in Figure~\ref{fig:midlines}.}: the Feuerbach and Jerabek Hyperbolas $F$ and $J$ \cite[Jerabek Hyperbola]{mw}. Both are rectangular since they contain $X_4$ \cite{mw}. The former is centered on $X_{11}$ and the latter on $X_{125}$. With respect to 3-periodics no invariants have been detected for $J$. However, the Jerabek $J_{exc}$ of the Excentral Triangle, which passes through the Excenters and is centered on $X_{100}$\footnote{The Excentral's $X_{125}$ \cite{mw}.}, does produce interesting invariants\footnote{The Feuerbach Hyperbola $F_{exc}$ has not yet yielded any detectable invariants over the 3-periodic family.}. 
$F$ is known to pass through $X_1$ and $X_9$ of its reference triangle. Interestingly
$J_{exc}$ also passes through $X_1$ and $X_9$. This stems from the fact that $J$ passes through $X_4$ and $X_6$. Since the Excentral Triangle is always acute \cite{coxeter67}, its $X_4$ is $X_1$. Likewise, the excentral $X_6$ is $X_9$. 

The Isogonal Conjugate of a Circumconic is a line \cite[Circumconic]{mw}. Remarkably:

\begin{remark}
The Isogonal conjugate of $F$ with respect to a reference triangle and that of $J_{exc}$ with respect to the Excentral one is line $X_1X_3=\mathcal{L}_{650}$.
\end{remark}

The first part is well-known \cite[Feuerbach Hyperbola]{mw}. For the second part, consider that $J$ is the Isogonal Conjugate of the Euler Line \cite[Jerabek Hyperbola]{mw}. The Euler Line of the Excentral Triangle passes through its $X_4$ and $X_5$ which are $X_1$ and $X_3$ in the reference 3-periodic.

Referring to Figure~\ref{fig:circumhyps}:

\begin{proposition}
$J_{exc}$ intersects $E_9$ in exactly two locations.
\end{proposition}

\begin{proof}
Let $s_i,i=1,2,3$ refer to 3-periodic sidelengths. The perspector of $J_{exc}$ is $X_{649}=s_1(s_2-s_3)::$ (cyclical) \cite{etc}. Therefore the trilinears $x:y:z$ of $J_{exc}$ satisfy \cite{yiu2003}:
 \[J_{exc}: {s_1(s_2-s_3)}x^2+s_2(s_3-s_1)y^2+s_3(s_1-s_2)z^2=0.\]
 
Notice the above is satisfied for the Excenters $[1:1:-1],\; [1:-1:1]$ and $ [-1:1:1]$. As $X_1=[1:1:1]$ and $X_9=s_2+s_3-s_1::$ (cyclical) it follows that
 $J_{exc}(X_1)=J_{exc}(X_9)=0$.
 
 Eliminating variable $x$, the intersection of $J_{exc}=0$ and $E_9=0$ is given by the quartic:
 
 \begin{align*}
 &s_2(s_1-s_3)k_1 y^4+2s_2(s_1-s_3){k_1}{k_2}y^3 z\\
 +&2s_3(s_1-s_2){k_1}{k_2}y z^3+s_3(s_1-s_2)k_1 z^4=0
 \end{align*}
 
With $k_1=(s_1+s_2-s_3)^2$ and $k_2=s_1+s_3-s_2$. The discriminant of the above equation is:
 
 \[
 -432[(s_2-s_3)(s_1-s_3)(s_1-s_2)(s_1+s_3-s_2)^2(s_1-s_2-s_3)^2(s_1+s_2-s_3)^2(s_1s_2s_3)]^2
 \]
 
Since it is negative, there will be two real and two complex solutions \cite{burnside_1960}.
\end{proof}



\begin{proposition}
$F$ intersects the $X_9$-centered Circumellipse at $X_{1156}$.
\end{proposition}

\begin{proof}
The perspector of $X_9$ is $X_1$ and that of $X_{11} $ is $X_{650}=(s_3-s_3)(s_3+s_3-s_1)::$ (cyclical). Therefore, the trilinears $x:y:z$ of $F$ and $E_9$ satisfy:

\begin{align*}
    F:&(s_2-s_3)(s_2+s_3-s_1)/x+\\
    &(s_3-s_1)(s_3+s_1-s_2)/y+\\
    &(s_1-s_2)(s_1+s_2-s_3)/z=0 \\
    E_9:& 1/x+1/y+1/z=0.
\end{align*} 

$X_{1156}$ is given by $1/[(s_2-s_3)^{2}+s_1( s_2+s_3-2s_1)]::$ (cyclic). This point can be readily checked to satisfy both of the above.
\end{proof}
 
 %abaixo: nao e a Jerabek do excentral e sim do bilhar
%The intersection of $E_9$ with the Jerabek circumhyperbola %$J$ is given by the point
%$X^*=[g(a,b,c):g(b,c,a):g(c,a,b)]$ where
%$g(a,b,c)=(b+c)(a^4 - ( b^2-bc+c^2)a^2-bc(b-c)^2)$. 

Given a generic triangle $T$, the following two claims are known:

\begin{proposition}
The asymptotes of both $F$ and $J_{exc}$ are parallel to the $X_9$-centered circumconic, i.e., $c_4$ and $c_5$ in \eqref{eqn:e0} vanish.
\end{proposition}

\begin{proof}
To see the first part, consider that since the Caustic is centered on $X_9$ and tangent to the 3-periodics, it is the (stationary) Mandart Inellipse $I_9$ of the family \cite{mw}. This inconic is known to have axes parallel to the asymptotes of $F$ \cite{gibert2004-mandart}. Since the Caustic is confocal with the EB, $F$ asymptotes must be parallel to the EB axes.

Secondly, 3-periodics are the Orthic Triangles of the Excentrals, therefore the EB is the (stationary) Excentral's Orthic Inconic \cite{mw}. The latter's axes are known to be parallel to the asymptotes of the Jerabek hyperbola. \cite[Orthic Inconic]{mw}.

An alternate, algebraic proof appears in Appendix \ref{app:circum-x1x2x9}.
\end{proof}

\noindent Let $\lambda$ (resp. $\lambda'$) be the focal length of $F$ (resp. $J_{exc}$).

\begin{remark}
Isosceles 3-periodics have $\lambda'=\lambda=0$.
\end{remark}

To see this consider the sideways isosceles 3-periodic with $P_1=(a,0)$. $P_2$ and $P_3$ will lie on the 2nd and 3rd quadrants at $(-a_c,{\pm}y')$, where $a_c=a(\delta-b^2)/(a^2-b^2)$ is the length of the Caustic major semi-axis \cite{garcia2020-ellipses}. $X_1$ and $X_4$ will lie along the 3-periodic's axis of symmetry, i.e., the x-axis. To pass through all 5 points, $F$ degenerates to a pair of orthogonal lines: the x-axis and the vertical line $x=-a_c$. The foci will collapse to the point $(-a_c,0)$. A similar degeneracy occurs for the upright isosceles, i.e., when $P_1=(0,b)$, namely, the foci collapse to $(0,-b_c)$, where $b_c=b(a^2-\delta)/(a^2-b^2)$ is the Caustic minor semi-axis length.

\begin{theorem}
For all non-isosceles 3-periodics, $\lambda'/\lambda$ is invariant and given by:
\label{thm:focal-ratio}
\end{theorem}
 
\begin{equation}
 \frac{\lambda'}{\lambda}=
 %\frac{\sqrt{\delta^2+\left(a^2+b^2\right)\delta+ a^2b^2}}{a b}
 \sqrt{2/\rho}>2
 \label{eqn:focal-ratio}
\end{equation}

\begin{proof}
Assume the EB is in the form of \eqref{eqn:billiard-f}. Let the 3-periodic be given by $P_i=(x_i,y_i),i=1,2,3$. $F$ passes through the $P_i$, $X_1$ and $X_9=(0,0)$. The asymptotes of $F$ are parallel to the EB axes, therefore this hyperbola is given by $c_1x+c_2y+c_3 x y = 0$ and $\lambda^2=|8c_1c_2/c_3^2|$, where: 
\begin{align}
c_1=& y_2y_3(x_2-x_3)x_1^2+(x_2^2y_3-x_3^2y_2-y_2^2y_3
+y_2y_3^2)x_1y_1 \nonumber\\
+&y_2y_3(x_2-x_3)y_1^2  
-(x_2y_3-x_3y_2)(x_2x_3+y_2y_3)y_1
 \nonumber \\
 c_2=&x_2x_3(y_2-y_3)x_1^2+(x_2x_3^2-x_2^2x_3-x_2y_3^2+x_3y_2^2)x_1y_1 \label{eqn:ci} \\
 +&(x_2y_3-x_3y_2)(x_2x_3+y_2y_3)x_1-x_2x_3(y_2-y_3)y_1^2 \nonumber\\
 c_3=& (x_2y_3-x_3y_2)x_1^2+
(x_3^2y_2-x_2^2y_3+  y_2^2y_3-y_2y_3^2)x_1 \nonumber\\
+&(x_3y_2-x_2y_3 )y_1^2 
+(x_2^2x_3-x_2x_3^2+x_2y_3^2-x_3y_2^2)y_1 \nonumber
\end{align}
 
Let $P_i'=(x_i',y_i'),i=1,2,3$ be the Excenters. They are given by
\begin{align} 
    P_1'=&\left({\frac {-{x_1}\,{s_1}+{x_2}\,{s_2}+{x_3}\,{s_3}}{{
s_2}+{s_3}-{s_1}}},{\frac {-{y_1}\,{s_1}+{y_2}\,{
s_2}+{y_3}\,{s_3}}{{s_2}+{s_3}-{s_1}}}\right) \nonumber\\
P_2'=& \left({\frac {{x_1}\,{s_1}-{x_2}\,{s_2}+{x_3}\,{s_3}}{{
s_3}+{s_1}-{s_2}}},{\frac {{y_1}\,{s_1}-{y_2}\,{
s_2}+{y_3}\,{s_3}}{{s_3}+{s_1}-{s_2}}}\right) \label{eqn:pi-prime} \\
P_3'=& \left({\frac {{x_1}\,{s_1}+{x_2}\,{s_2}-{x_3}\,{s_3}}{{
s_1}+{s_2}-{s_3}}},{\frac {{y_1}\,{s_1}+{y_2}\,{
s_2}-{y_3}\,{s_3}}{{s_1}+{s_2}-{s_3}}}\right) \nonumber
\end{align}
Here, $s_1=|P_2-P_3|$, $s_2=|P_1-P_3|$ and $s_3=|P_1-P_2|$.

Since $J_{exc}$ is also centered on the origin and has horizontal/vertical asymptotes, $J_{exc}$ is given by $c_1'x+c_2'y+c_3'x y=0$, and $(\lambda')^2=|8c_1'c_2'/(c_3')^2|$, where $c_i'$ are constructed as \eqref{eqn:ci} replacing $(x_i,y_i)$ with $(x_i',y_i')$.

Consider a right-triangle\footnote{We found this to best simplify the algebra.} 3-periodic, e.g., with $P_1$ at $(x^\perp,y^\perp)$ given in \eqref{eqn:perp} and $P_2$ and $P_3$ obtained explicitly \cite{garcia2019-incenter}. From these obtain $c_i$ using \eqref{eqn:ci}. Using \eqref{eqn:pi-prime} obtain $P_i'$ and the $c_i'$. Finally, obtain a symbolic expression for $\lambda'/\lambda$. After some manipulation and simplification with a Computer Algebra System (CAS), we obtain \eqref{eqn:focal-ratio} which we call a {\em candidate}.

Parametrize the 3-periodic family with $P_1(t)=(a\cos{t},b\sin{t})$ and using the sequence above arrive at an expression for $\lambda'/\lambda$ in terms of $t$. Subtract that from the right-triangle candidate. After some algebraic manipulation and CAS simplification verify the subtraction vanishes, i.e., $\lambda'/\lambda$ is independent of $t$.
\end{proof}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0060_circumhyps.eps}
    \caption{An $a/b=1.5$ EB is shown (black) as well as a sample 3-periodic (blue), the confocal Caustic (brown), and the Excentral Triangle (green). The 3-periodic's Feuerbach Circumhyperbola $F$ (orange) passes through its three vertices as well as $X_1$, $X_9$, and $X_4$. The Excentral's Jerabek Circumhyperbola $J_{exc}$ (purple) passes through the three Excenters, as well as $X_1$, $X_9$ and $X_{40}$ (not shown). Two invariants have been detected over the orbit family: (i) the asymptotes (dashed) of both $F$ and $J_{exc}$ stay parallel to the EB axes, (ii) the ratio of focal lengths is constant (focal axis appears dashed). $F$ intersects the Billiard at $X_{1156}$.}
    \label{fig:circumhyps}
\end{figure}

\subsection{Focal Length Extrema}

Let $P_1(t)=(a\cos{t},b\sin{t})$. While their ratio is constant, $\lambda$ and $\lambda'$ undergo three simultaneous maxima in $t\in(0,\pi/2)$, see Figure~\ref{fig:focal-ratio}. In fact, the following additional properties occur at configurations of maximal focal length (we omit the rather long algebraic proofs), see Figure~\ref{fig:zero-hyps}:

\begin{itemize}
    \item $F'$ is tangent to the Caustic at ${\pm}X_{11}$.
    \item $J'_{exc}$ is tangent to the EB at ${\pm}X_{100}$, i.e., at ${\mp}X_{1156}$ (see below).
    %\item $k'_J=a/b$.
\end{itemize}

\begin{remark}
Like $F$, $J'_{exc}$ intersects the EB at $X_{1156}$.
\end{remark}

This happens because $X_{1156}$ is the reflection of $X_{100}$ about $X_9$. If the latter is placed on the origin, then $X_{1156}=-X_{100}$, and $J'_{exc}$ passes through ${\pm}X_{100}$.

Let $F'$ and $J'_{exc}$ be copies of $F$ and $J_{exc}$ translated by $-X_{11}$ and $-X_{100}$ respectively, i.e., they become concentric with the EB (focal lengths are unchanged). Since their asymptotes are parallel to the EB axes and centered on the origin, their equations will be of the form:

\[
F': x\,y = k'_F,\;\;J'_{exc}: x\,y = k'_J
\]

\begin{remark}
$\lambda=2\sqrt{2k'_F}$, $\lambda'=2\sqrt{2k'_J}$, $\lambda'/\lambda=\sqrt{k'_J/k'_F}=\sqrt{2/\rho}$.
\end{remark} 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0110_hyp_focals.eps}
    \caption{Focal lengths $\lambda,\lambda'$ of $F,J_{exc}$ vs the parameter $t$ in $P_1(t)=(a\cos{t},b\sin{t})$ are shown red and green. The solid (resp. dasheD) curves correspond to $a/b=1.5$ (resp. $a/b=1.3$). In the first quadrant there are 3 maxima. $\lambda'/\lambda$ (blue) remain constant for the whole interval.}
    \label{fig:focal-ratio}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics_eps_new/0100_zero_hyps.eps}
    \caption{Two snapshots of $J$ and $F_{exc}$ drawn solid blue and solid green, respectively, for $a/b=1.5$. Also shown (dashed) are copies $F'$ and $J'_{exc}$ of both hyperbolas translated so they are dynamically concentric with the EB (translate $J$ by $-X_{11}$ and $F_{exc}$ by $-X_{100}$). Their focal lengths $\lambda,\lambda'$ are identical to the original ones; their focal axes are collinear and shown the dashed diagonal through the EB center. Notice that like $F$, $J'$ also intersects the EB at $X_{1156}$. \textbf{Left}: $t=10.1^\circ$, showing an intermediate value of ether focal length. \textbf{Right}: $t=6.2^\circ$, focal lengths are at a maximum. When this happens, the translated copy of $F$ (resp. $J_{exc}$) is tangent to the Caustic (resp. EB) at $X_{11}$ (resp. $X_{1156})$. \textbf{Video}: \cite[PL\#09,10]{reznik2020-playlist-circum}}
    \label{fig:zero-hyps}
\end{figure}

\

==> _not_used/070_inconics.tex <==
A triangle's {\em Inconic} touches its three sides while satisfying two other constraints, e.g., the location of its center. Similar to Circumconics, if the latter is interior to the 4 shaded regions in  Figure~\ref{fig:midlines} it is an ellipse, else it is a hyperbola. Lines drawn from each vertex to the Inconic tangency points concur at the perspector or Brianchon Point $B$ \cite{mw}.

Let the Inconic center $C$ be specified by Barycentrics\footnote{Barycentrics $g$ can be easily converted to Trilinears $f$ via: $f(s_1,s_2,s_3)=g(s_1,s_2,s_3)/s_1$ (cyclic) \cite{yiu2003}.} $g(s_1,s_2,s_3)$ (cyclic), then $B$ is given by $1/[g(s_2,s_3,s_1)+g(s_3,s_1,s_2)-g(s_1,s_2,s_3)]$ (cyclic) \cite{stothers2001-circumconics}. For example, consider the Inconic centered on $X_1$ (the Incircle), i.e., $g=s_2 s_3$ (cyclic). Then $B=1/(s_1 s_3+s_1 s_2-s_2 s_3)$. Dividing by the product ${s_1}{s_2}{s_3}$ obtain $B=1/(s_2 + s_3 - s_1)$ (cyclic), confirming that the perspector of the Incircle is the Gergonne Point $X_7$ \cite[Perspector]{mw}. The contact points are the vertices of the Cevian triangle through $B$.

Above we identified the confocal Caustic with the Mandart Inellipse $I_9$ \cite{mw} of the 3-periodic family, i.e., it is a stationary ellipse centered on $X_9$ and axis-aligned with the EB, Figure~\ref{fig:three-orbits-proof}. Its semi-axes $a_c,b_c$ are given by \cite{garcia2019-incenter}:

\begin{equation*}
a_c=\frac{a\left(\delta-{b}^{2}\right)}{a^2-b^2},\;\;\;
b_c=\frac{b\left({a}^{2}-\delta\right)}{a^2-b^2}\cdot
\end{equation*}

Similarly, the $X_9$-centered Inconic of the family of Excentral Triangles is the stationary EB, i.e., the EB is the Orthic Inconic \cite{mw} of the Excentrals.

\subsection{Excentral $X_3$-Centered Inconic}

No particular invariants have yet been found for any of the Inconics to 3-periodics with centers in $X_i$, $i=3,4,\ldots,12$. Let $I_3$ denote the $X_3$-centered inconic. Its Brianchon Point is $X_{69}$ and its foci aren't named centers \cite{moses2020-private-circumconic}.

\begin{remark}
$I_3$ is always an ellipse.
\end{remark}

To see this consider the Circumcenter of an acute, right, or obtuse triangle lies inside, on a vertex, or opposite to the interior of the Medial, respectively, i.e., within one of the 4 shaded regions in Figure~\ref{fig:midlines}.

Let $I'_3$ denote the $X_3$-centered Inconic of the Excentral Triangle. Its Brianchon Point is $X_{69}$ of the Excentral, i.e., $X_{2951}$ of the reference 3-periodic \cite{moses2020-private-circumconic}, Figure~\ref{fig:macbeath-excentral}(left). Let $\mu'_3,\mu_3$ denote $I_3'$ major and minor semi-axes. In \cite{reznik2020-poristic} we show:

\begin{proposition}
Let $T$ be a triangle and $T'$ its excentral. The Inconic $I_3'$ to $T'$ on its Circumcenter ($X_{40}$ of $T$) is a $90^\circ$-rotated copy of the $E_1$, the $X_1$-centered Circumconic, i.e.:

\begin{equation}
\mu_3'= \eta_1',\;\;\;\mu_3=\eta_1
\end{equation}
\end{proposition}

\begin{figure}
    \centering    \includegraphics[width=\textwidth]{pics_eps_new/0150_two_inconics.eps}
    \caption{\textbf{Left}: The $X_{3}$-centered Inconic $I_3'$ (red) of the Excentral Triangle (green), whose center is $X_{40}$ in terms of the 3-periodic (blue). Its Brianchon Point is $X_{2951}$ \cite{moses2020-private-circumconic}. Its axes are aligned with the EB which it intersects at $X_{100}$, and its aspect ratio is invariant. The $X_1$-centered Circumconic $E_1$ (green) is a $90^\circ$-rotated copy of $I_3'$. \textbf{Right}: The MacBeath Inconic $I_5'$ of the Excentral (red) is centered on the latter's $X_5$ and has foci on $X_4$ and $X_3$. These correspond to  $X_3$, $X_1$, and $X_{40}$ of the reference triangle (blue). Its Brianchon Point is $X_{1742}$ \cite{moses2020-private-circumconic}. Though its axes are askew with respect to the EB, its aspect ratio is invariant over the 3-periodic family. \textbf{Video}: \cite[PL\#11]{reznik2020-playlist-circum}.}
    \label{fig:macbeath-excentral}
\end{figure}

\begin{remark}
As $E_1$, $I'_3$ is axis-aligned with the EB and contains $X_{100}$, Figure~\ref{fig:macbeath-excentral} (left).
\end{remark}

\begin{theorem}
Over 3-periodics, $\mu_3'$ and $\mu_3$ are variable though their ratio is invariant. These are given by:

\begin{align*}
\mu_3'=&R+d,\;\;\;\mu_3=R-d\\
\frac{\mu_3'}{\mu_3}=&
%\frac{\sqrt{2\delta(\delta+ a^2 - b^2) - a^2 b^2}}{b^2}
\frac{R+d}{R-d} = \frac{1+\sqrt{1-2\rho}}{\rho}-1>1
\end{align*}
\label{thm:excIncX3}
\end{theorem}

\noindent As above, $d=\sqrt{R(R-2r)}$, and $\rho=r/R$.

\begin{proof}
The above was initially a candidate an isosceles 3-periodic and then verified it held any 3-periodic configuration with a CAS. A related proof appears in \cite{reznik2020-poristic}.
\end{proof}

\subsection{Excentral  X$_5$-Centered (MacBeath) Inconic}

Above the locus of the Excenters is identified with the Excentral MacBeath Circumconic $E_6' $. The MacBeath {\em Inconic} $I_5$ of a triangle is centered on $X_5$ and has foci on $X_4$ and $X_3$. Its Brianchon Point is $X_{264}$, and it can be both an ellipse or a hyperbola \cite[MacBeath Inconic]{mw}. No invariants have yet been found for $I_5$.

Consider $I'_5$, the MacBeath Inconic of the Excentral Triangle, Figure~\ref{fig:macbeath-excentral}(right). The center and foci of $I'_5$ with respect to the reference triangle are $X_3$, $X_1$, and $X_{40}$, respectively, and its Brianchon is $X_{1742}$ \cite{moses2020-private-circumconic}. Unlike $I'_3$, the axes of $I'_5$ are askew with respect to the EB.

\begin{remark}
$I'_5$ is always an ellipse.
\end{remark}

This is due to the fact that the Excentral is acute as is its homothetic Medial. Since $X_5$ is the latter's Circumcenter, it must lie inside it.

\noindent Let $\mu'_5,\mu_5$ denote $I_5'$ major and minor semi-axes.

\begin{theorem}
Over the 3-periodic family $\mu_5'$ and $\mu_5$ are variable and their ratio is invariant. These are given by:

\begin{align*}
\mu_5'=&R,\;\;\;\mu_5=\sqrt{R^2-d^2}\\
 \frac{\mu_5'}{\mu_5}=&\frac{R}{\sqrt{R^2-d^2}}=\frac{1}{\sqrt{2 \rho}}\\
 %=&\frac {\left( {b}^{2}+\delta \right) \sqrt {\delta+{a}^{2}-{b}^{2} } }{2b{a}^{2}}
 %= \frac {\left({a}^{2}+\delta\right) \sqrt {\delta+{b}^{2}-{a}^{2}} }{2a{b}^{2}}
\end{align*}
\label{thm:excIncX5}
\end{theorem}

The above was derived for an isosceles 3-periodic and shown to work for any $a,b$. A related proof is given in \cite{reznik2020-poristic}.


==> _not_used/099_pythagorean.tex <==
We have seen \cite{ronaldo2020-loci} that with $a/b>a_4=\sqrt{2\,\sqrt{2}-1}\simeq{1.352}$ the orbit family contains obtuse triangles amongst which there always are 4 right triangles (identical up to rotation and reflection). An interesting question is which EB aspect ratios produce primitive {\em Pythagorean} triangles, i.e., right triangles with sides $s_1,s_2,s_3$ for which $s_1,s_2$ are co-prime, and $s_3^2=s_1^2+s_2^2$.

Start with an elementary Pythagorean triangle $P_1=(0,0)$, $P_2=(s_1,0)$, and $P_3=(s_1,s_2)$ choosing $s_1,s_2$ integers such that $s_3=s_3=\sqrt{s_1^2+s_2^2}$ is an integer.
The Circumbilliard is given by
\[
E_9(x,y)= s_2 x^2+ \left( s_3-s_1-s_2 \right) xy+s_1{y}^{2}-s_1s_2x-s_1 \left( s_1-s_3 \right) y=0.\]

Computing the axes of its Circumbilliard we obtain: 

\begin{equation}
    [a/b](s_1,s_2,s_3)= \frac {s_1+s_2+\sqrt {s_3\left(3\,s_3-2\,s_1-2\,s_2\right) }}{\sqrt { \left( 
s_1+s_2+3\,s_3 \right)  \left( s_1+s_2-s_3 \right) }}
\end{equation}

%\begin{equation*}
  %  \lim_{s_2\to \infty} %r(s_2,s_2,\sqrt{2}s_2)=\sqrt{2\sqrt{2}-1}\simeq %1.352
%\end{equation*}
%The axis of the Circumbilliard are:

%\begin{align}
%    a(m,n,p)=&  \\
 %   b(m,n,p)=&
%\end{align}

Table~\ref{tab:pythagorean} shows the aspect ratios required for the first 16 Pythagorean triples ordered by hypotenuse\footnote{The $a/b$ which produces $3:4:5$ was first computed in \cite{ronaldo2020-loci} in connection with $X_{88}$.}

\begin{table}[H]
\scriptsize
$$
\begin{array}{r|c|l|l}
(s_1,s_2,s_3) & a/b & {\simeq}a/b & \text{isosc. rank} \\
\hline
3, 4, 5 & {(7+\sqrt{5})\sqrt{11}}/{22} &  1.392 &  4 \\
5, 12, 13 & {\sqrt{14} (\sqrt{65}+17)}/{56} & 1.674 &  10 \\
8, 15, 17 & {\sqrt{111} (\sqrt{85}+23)}/{222} & 1.529 & 8\\
7, 24, 25  & {\sqrt{159} (5\,\sqrt{13}+31)}/{318} & 1.944 & 12 \\
\mathbf{20, 21, 29} & \mathbf{\sqrt{6} (\sqrt{145}+41)/{96}} & \mathbf{1.353} &  \mathbf{1} \\
12, 35, 37 & {\sqrt{395} (\sqrt{629}+47)}/{790} & 1.813 & 11 \\
9, 40, 41 & {\sqrt{86} (5\,\sqrt{41}+49)}/{344}& 2.184 &  14 \\
28, 45, 53 & {\sqrt{290} (\sqrt{689}+73)}/{1160} & 1.457 & 5 \\
11, 60, 61 & {\sqrt{635} (\sqrt{2501}+71)}/{1270} & 2.401 & 15 \\
16, 63, 65 & {\sqrt{959} (\sqrt{2405}+79)}/{1918} & 2.067 & 13 \\
33, 56, 65 & {\sqrt{426} (\sqrt{1105}+89)}/{1704} & 1.481  & 6 \\
48, 55, 73 & {\sqrt{2415} (\sqrt{949}+103)}/{4830} & 1.361 &  3 \\
\mathbf{13, 84, 85} & \mathbf{\sqrt{66} (97+\sqrt{5185})/{528}} & \mathbf{2.600} & \mathbf{16} \\
36, 77, 85 & {\sqrt{161} (\sqrt{2465}+113)}/{1288} & 1.602 & 9 \\
39, 80, 89 & {\sqrt{2895} (\sqrt{2581}+119)}/{5790} & 1.578 &  8 \\
65, 72, 97 & {\sqrt{1070} (\sqrt{1649}+137)}/{4280}& 1.357 & 2
\end{array}
$$
%\[a/b_{\perp}(m,n,p)=\sqrt {{\frac {m+n+\sqrt {p %( -2\,m-2\,n+3\,p \right) }}{m+n-
%\sqrt {p ( -2\,m-2\,n+3\,p \right) }}}}\]
\caption{The first column shows the first 16 Pythagorean triples ordered by hypotenuse $s_3$. The second one shows the $a/b$ family which produces it. The boldfaced triple $(20,21,29)$ (resp.~$(13,84,85)$) is the closest (resp.~farthest) to an isosceles in the table. This means $a/b$ will be closest to $a_4=1.352$. If rows were listed in ascending order of  $|s_1/s_2-1|$ (how scalene a triple is), the values of $a/b$ would also appear ascending, as indicated by the ``rank'' column.}
\label{tab:pythagorean}
\end{table}
%


\subsection{First 12k Pythagoreans in $a,b$ space}

Euclid's Algorithm generates a primitive Pythagorean triple from a co-prime pair $m,n$, $m>n$. For example, $(3,4,5)$ (resp.~$(5,12,13)$) is generated with $m=2,n=1$ (resp., $m=3,n=2$), etc.

Figure~\ref{fig:pythagorean} shows the first 12231 triangles generated in this fashion with $1<m<200$ in both $(s_1,s_2)$ and $(a,b)$ space. A few interesting observations are given in the caption. 

\begin{figure}[H]
    \centering
    \includegraphics[width=\textwidth]{pics_eps/0101_pythagorean_legs_ab.eps}
    \caption{\textbf{Top}: Right-triangles generated by Euclid's Algorithm with $n<m<200$, $m,n$ co-prime. Roughly 12k $(s_1,s_2)$ leg combinations are shown as black dots. To save space, the y-axis is drawn half-scale and points with $s_2>50000$ are not drawn. The green line represents $s_1=s_2$, i.e., isosceles triangles (only quasi-isosceles can be generated). The red (resp.~blue) curve is drawn over triangles obtained with $m=150$ (resp.~$n=150$). \textbf{Bottom}: Axes $(a,b)$ combinations which can produce the aforementioned right-triangles. The point cloud is properly under the green line $a/b=a_4$ (aspect ratio which produces an isosceles right-triangle). The constant $m=150$ (resp.~$n=150$) runs produce a red (resp.~blue) arch in $(a,b)$ space. Quasi-similar triangles organize in straight lines from the origin toward the right, i.e., they are generated by quasi-similar billiards.}
    \label{fig:pythagorean}
\end{figure}

\subsection{Iso-perimetric Primitive Pythagoreans}

Out of the 12231 Pythagorean triples generated, only 11548 perimeters $s_1+s_2+s_3$ are unique. Out of these, 10912 are associated with a single triple. An additional 585 (resp.~47) unique perimeters are each produced by two (resp.~3) distinct triples. Finally, 2 unique perimeters -- 60060 and 78540 -- are shared by two distinct groups of four triples, listed below:

$$
\scriptsize
\begin{array}{|c|c|c|c|}
\hline
\text{L} & s_1 & s_2 & s_3 \\
\hline
 60060 & 6699 & 26260 & 27101 \\
 60060 & 15960 & 19162 & 24938 \\
 60060 & 22035 & 12628 & 25397 \\
 60060 & 26936 & 5610 & 27514 \\
 78540 & 13515 & 31108 & 33917 \\
 78540 & 21896 & 24090 & 32554 \\
 78540 & 25179 & 20740 & 32621 \\
 78540 & 34440 & 8602 & 35498 \\
 \hline
\end{array}
$$

The perimeter $L$ of a 3-periodic orbit as a function of the EB axes $a,b$ is given by \cite{ronaldo2020-loci}:

\begin{equation*}
L=\frac{2(\delta+a^2+b^2)\sqrt{2\delta-a^2-b^2}}{a^2-b^2}
\end{equation*}

\noindent with $\delta=\sqrt(a^4-a^2 b^2+b^4)$. Each $L$ defines a level curve in $(a,b)$ space\footnote{Given by the quartic $(a^2-b^2)^2 L^4-(2(2a^2-b^2))(a^2-2 b^2)(a^2+b^2) L^2-27 a^4 b^4=0$.} which represents a 1d family of EBs such that all their orbit families have the same perimeter, see Figure~\ref{fig:iso-perimeter-3-and-4}.

The two groups of 4 triples with the same perimeter are shown in Figure~\ref{fig:iso-perimeter-4} against level curves of their perimeter. A similar picture for the 4-groups and 3-groups is shown in Figure~\ref{fig:iso-perimeter-3-and-4}.

\begin{figure}[H]
    \centering
    \includegraphics[width=.66\textwidth]{pics_eps/0120_fourTriplesPlot.eps}
    \caption{Two iso-perimetric curves are shown in $(a,b)$ space corresponding to EB families whose orbits have the same perimeter. Also shown are the 4-member groups of primitive Pythagorean triples sharing either perimeter.}
    \label{fig:iso-perimeter-4}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=.66\textwidth]{pics_eps/0121_fourTriplesAllPlot}
    \caption{All 4- and 3-groups of Pythagorean triples with the same perimeter. They fall on common iso-perimeter level curves (red) in $(a,b)$ space.}
    \label{fig:iso-perimeter-3-and-4}
\end{figure}

==> _not_used/102_app_orbit_vertices.tex <==
Let the boundary of the Billiard satisfy Equation~\eqref{eqn:billiard-f}. Assume, without loss of generality, that $a{\geq}b$.

Given a starting vertex $P_1$ and an exit angle $\alpha$ (as above), the orbit $P_1P_2P_3$ will be such that \cite{ronaldo19}:

vertex $P_2$ will be given by $(p_{2x},p_{2y})/q_2$, with

\begin{align*}
%\label{eqn:p2}
p_{2x}=&-{b}^{4} \left(  \left(   a^2+{b}^{2}\right)\cos^{2}\alpha   -{a}^{2}  \right) x_1^{3}-2\,{a}^{4}{b}^{2} \cos \alpha  \,\sin  \alpha  \,  x_1^{2}{y_1}\\
&+{a}^{4} \left(  ({a
}^{2}-3\, {b}^{2}) \cos^{2} \alpha  +{b}^{2}
 \right) {x_1}\,y_1^{2}-2{a}^{6} \,\cos  \alpha  \sin   \alpha  \, y_1^{3} ,
\\
p_{2y}=& 2{b}^{6} \,\cos \alpha\sin \alpha\,   x_1^{3}+{b}^{4}\left(  ({b
 }^{2}-3\, {a}^{2}) \cos^{2} \alpha  +{a}^{2}
  \right) x_1^{2}{y_1}\\
&+  2\,{a}^{2} {b}^{4}\cos \alpha \sin
  \alpha \; {x_1} y_1^{2} -{
a}^{4}  \left(  \left(   a^2+{b}^{2}\right)\cos^{2}  \alpha  -{b}^{2}  \right)  y_1^{3}
\\
q_2=&{b}^{4} \left( a^2-c^2\cos^2\alpha   \right)
x_1^{2}+{a}^{4} \left(  {b}^{2}+c^2\cos^2 \alpha  
 \right) y_1^{2}\\
 & - 2\, {a}^{2}{b}^{2}{c^2}\cos \alpha\sin \alpha \; {x_1}\,{
y_1}.
\end{align*}

and vertex $P_3$ will be given by $(p_{3x},p_{3y})/q_3$, with:

\begin{align*}
p_{3x}=& {b}^{4} \left( {a}^{2}- \left( {b}^{2}+{a}^{2} \right) \right)
 \cos^{2}  \alpha   x_1^{3} +2\,{a}^{4}{b}^{2} \cos  \alpha \sin \alpha\,   x_1^{2}{ y_1}\\
 &+{a}^{4} \left( 
  \cos^{2}  \alpha  \left( {a}^{2}-3\,{b}^{2}
 \right) +{b}^{2} \right) { x_1}\, y_1^{2} +2\, {a}^{6} 
 \cos \alpha\,\sin \alpha\, y_1^{3}
\\
p_{3y}=& -2\, {b}^{6} \cos \alpha\sin \alpha\, x_1^{3}+{b}^{4} \left( {a}^{2}+ \left( {b}^{2}-3\,{a}^{2} \right)    \cos^2\alpha \right) {{ x_1}}^{2}{ y_1}
\\
& -2\,{a}^{2}  {b}^{4}\cos
 \alpha  \sin \alpha\,  x_1 y_1^{2}+
 {a}^{4} \left( {b}^{2}- \left( {b}^{2}+{a}^{2} \right)   \cos^{2}  \alpha  \right)\,  y_1^{3},
\\
q_3=& {b}^{4} \left( {a}^{2}-{c^2}\cos^{2}\alpha   \right) x_1^{2}+{a}^{4} \left( {b}^{2}+c^2\cos^{2}\alpha  \right)  y_1^{2}\\
&+2\,{a}^{2}{b}^{
2} c^2 \cos\alpha \sin\alpha\, { x_1}\,{ y_1}.
\end{align*}

The sides of the triangular orbit have lengths 
$s_1=\mid P_3-P_2\mid$, $s_2=\mid P_3-P_1\mid$ and
$s_3=\mid P_2-P_1\mid$.

==> _not_used/104_app_circumellipses_X1X2X9.tex <==
Let a triangle $T$ have vertices $P_1=(0,0)$, $P_2=(1,0)$ and $P_3=(u,v)$ and sidelengths $s_1,s_2,s_3$. Using the linear system in Appendix~\ref{app:circum-linear}, one can obtain implicit equations for the circumellipses $E_9,E_1,E_2$ centered on $T$'s Mittenpunkt $X_9$, Incenter $X_1$, and Barycenter $X_2$, respectively:

\begin{align*}
E_9(x,y)=&  v^2 x^2-v(s_1 -s_2-1+2u)xy+((s_1-s_2-1)u+u^2+s_2 )y^2\\
-&v^2x+((s_1-s_2-1)u+u^2+s_2)y^2+v(u-s_2)y=0\\
%
E_1(x,y)=&  \left( L-2 \right) {v}^{2}{x}^{2} + \left( L-2\,{ s_2}-2\,u
 \right)   \left( L-2 \right) v\, xy \\
 +& \left( 
-{L}^{2}u+ \left( 2\,u+1 \right) L{ s_2}+ \left( {u}^{2}+2\,u
 \right) L-2\,{s_2}^{2}-4\,u{ s_2}-2\,{u}^{2} \right) {y}^{2}\\
 -& \left( L-2 \right) {v}^{2} x
 - v\left( L{ s_2}-uL-2\,{s_2}^{2}+2\,u \right) y 
\\
E_2(x,y)=&v^2x^2+v(1-2u)xy+(u^2-u+1)y^2-v^2x+v(u-1)y=0\\
s_1=& \sqrt{(u-1)^2+v^2},\;\;\; s_2=\sqrt{u^2+v^2}, \;\;\; L=s_1+s_2+1
\end{align*}

Consider the quadratic forms
\begin{align*}
    q_9(x,y)=&   v\left(  { s_1}\, -{ s_2}\, +2 u  -1 \right) {x}^{2}+ 2\left(  (s_2-s_1)u
 - { s_2} - \,{u}^{2}+ u+  {v}^{2}
 \right) xy\\
 +& v\left( 1-2u - { s_1}\, +{ s_2}\,    \right) {y}^{2}
 \\
 q_1(x,y)=& -v \left( L-2 \right)  \left( L-2\,{ s_2}-2\,u \right) {x}^{2}+v  \left( L-2 \right)  \left( L-2\,{ s_2}-2\,u\right)y^2 \\
 +&
2 (  L^2u-(2u+1)Ls_2+(v^2-u^2-2u)L+ 4s_2u+4u^2 ) xy\\
q_2(x,y)=&v(2u+1)x^2+2(-u^2+v^2+u-1)xy+v(1-2u)y^2
\end{align*}

The axes of $E_9$ (resp. $E_1$) are defined by the zeros of $q_9$ (resp. $q_1$). Using the above equations it is straightforward to show that the axes of $E_1$ and $E_9$ are parallel.

The axes of $E_2$ and $E_9$ are parallel if and only if $(u-1)^2+v^2=1$ or $u^2+v^2=1$; this means that the triangle is isosceles.

The implicit equations of the circumhyperbolas $F $ passing through the vertices of the orbit centered on $X_{11}$ and   $J_{exc} $ passing through the vertices of the excentral triangle and centered on $X_{100}$ are:
{\small 
\begin{align*}
F(x,y)=& v^3(2 u  -1) (x^2-y^2)+  v^3(1-2u)x\\
+&[( s_2^3+(u-1) s_2^2-u s_2) s_1+(2u-1)s_2^2-us_1^2s_2 -u^4-4 u^2 v^2+v^4+2 uv^2] x y\\
 +&[ s_1^2 u^2  s_2+(-u  s_2^3-u (u-1)  s_2^2+ s_2 u^2)  s_1+u  s_2^4-v^2  s_2^2-u^3 (2 u-1)]y=0\\
 J_{exc}(x,y)=&  4v^3\left( 2\,u -1\, \right) ({x}^{2}-y^2)\\
 +& [ \left( 4\,s_2^{3}+ 4\left(  u-1
 \right)     s_2 ^{2}-4\,u{   s_2} \right) {   s_1}  -4\,u 
   s_1 ^{2}{   s_2} -4\,    s_2 ^{2} \\
   -&4\,{u}^{4}-16\,{
u}^{2}{v}^{2}+4\,{v}^{4}+8\,{u}^{3}+16\,u{v}^{2}
 ] xy\\
 +&[ (2 (- s_1  s_2^3+( (1- s_1) u-v^2+ s_1)  s_2^2+u  s_1 ( s_1+1)  s_2+u (u-2) s_1^2)) v]x\\
 +&[ (4-4 u) s_2  ((u^2-( \frac{1}{2} s_1 +1) u+ \frac{1}{2} s_1 +\frac{1}{2}) s_2 + \frac{1}{2} u s_1  (s_1 +1)- \frac{1}{2} s_2 ^2 (s_2 +s_1 ))]y\\
   -& u  s_1^2 v  s_2+(v  s_2^3+(-1+u) v  s_2^2-u v  s_2)  s_1+v  s_2^4-(2 u^2-2 u+1) v  s_2^2=0
\end{align*}
}
 Using the above equations it is straightforward to show that the axes of $E_9$ and asymptotes  of $F $ and $J_{exc} $ are parallel.

==> _not_used/105_app_ce_parallel.tex <==
Consider a triangle with vertices $A=(u,v)$, $B=(-1,0)$ and $C=(1,0).$ Let $s_2=|A-B|$ and $s_3=|B-C|$.
The equation of $F_{med}$ is given by:
{\small  
\begin{equation}    
\aligned 
F_{med}(x,y)=&4 u v^3(x^2- y^2) (2( u-1)  s_3  s_2^2-( 2(u-1)  s_3^2-2( u^2+ v^2-1) s_3)s_2\\ 
&2(u^2-1)^2+2v^2(4u^2-v^2)) xy\\
&+(-((u^2+v^2-1)  s_3+ s_3^2 (u-1)) v  s_2+ s_2^2 (u+1) v  s_3\\
-& v(v^4+(u^2-1)^2 ) x\\
+&(2 u^2+2 v^2-2)   u v^2\; y=0
\endaligned
\end{equation}
}
A one parameter family of circumellipses passing through $A$, $B$, $C$ and $X_{100}$ is given by:

\begin{equation}\aligned  
 E_b(x,y)
 =&  u v^3(bxy  -4  x^2)\\
 + &((b (u^2+v^2-1)  s_3+b (u-1)  s_3^2)  s_2-b (u+1)  s_2^2  s_3\\
 -&v^2(b(4u^2-v^2)+4uv)-b(u^2-1)^2) y^2\\ 
 -&v ((b (u^2+v^2-1)  s_2-b (u+1)  s_2^2)  s_3+b (u-1)  s_3^2  s_2\\
-&b(u^2+v^2-1) (  u^2-  v^2+  u v-1)) y+ 4 u v^3=0
 \endaligned
\end{equation}

It is
straightforward to verify that the family $E_b$ is
axis aligned (independent of b). Denoting the center of $E_b$ by $(x_c,y_c)$ it follows, using CAS, that $F_{med}(x_c,y_c)=0.$

The reciprocal
follows similarly.
